Contextual Metaprogramming for Session Types

We propose the integration of staged metaprogramming into a session-typed message passing functional language. We build on a model of contextual modal type theory with multi-level contexts, where contextual values, closing arbitrary terms over a series of variables, may be boxed and transmitted in messages. Once received, one such value may then be unboxed and locally applied before being run. To motivate this integration, we present examples of real-world use cases, for which our system would be suitable, such as servers preparing and shipping code on demand via session typed messages. We present a type system that distinguishes linear (used exactly once) from unrestricted (used an unbounded number of times) resources, and further define a type checker, suitable for a concrete implementation. We show type preservation, a progress result for sequential computations and absence of runtime errors for the concurrent runtime environment, as well as the correctness of the type checker.

==> packages/macros-content-toggles.tex <==
%% Macros for content toggles

% Toggle meta contents, such as todo lists, lists of typos, etc
\newtoggle{meta-contents}
\toggletrue{meta-contents}

% Toggle todo-notes
\newtoggle{todo-notes}
\toggletrue{todo-notes}

% Hide abbreviated proofs: \prooftrue to show; \prooffalse to hide
\newif\ifproof
\prooftrue

% Show technical report only contents
%\newif\iftechnical
%\technicaltrue

% Show submission only contents
%\newif\ifsubmission
%\submissionfalse


==> packages/macros-notation.tex <==
%% Macros for notation used in the system


%% GENERAL MACROS

\newcommand{\keyword}[1]{\mathsf{#1}}

%%% Grammar Macros
\newcommand{\grammarEq}{::=}
\newcommand{\grammarOr}{\mid}

%%% Substitutions
\newcommand{\substitution}[2]{[#1/#2]} % conventional

%% TYPES

%%% Type Meta Variables
\newcommand{\modeOp}{{\ensuremath{\sharp}}}
\newcommand{\sendOp}{{!}}
\newcommand{\receiveOp}{{?}}

\newcommand{\choiceOp}{{\ensuremath{\astrosun}}}
\newcommand{\internalChoiceOp}{{\ensuremath{\oplus}}}
\newcommand{\externalChoiceOp}{{\ensuremath{\&}}}

%%% Base types
\newcommand{\Unit}{{\keyword{Unit}}}
\newcommand{\Int}{{\keyword{Int}}}
\newcommand{\Bool}{{\keyword{Bool}}}
\newcommand{\Char}{{\keyword{Char}}}

%%% Session Types
\newcommand{\Skip}{{\keyword{Skip}}}
\newcommand{\Wait}{{\keyword{Wait}}}
\newcommand{\Close}{{\keyword{Close}}}
\newcommand{\modeType}[3]{{\ensuremath{#1 #2 . #3}}}
\newcommand{\choiceType}[3]{{\ensuremath{#1 \{#2\}^{#3}}}}
\newcommand{\recursiveType}[2]{{\ensuremath{\mu #1 . #2}}}

%%% Functional Types
\newcommand{\functionType}[2]{{\ensuremath{#1 \rightarrow #2}}}
\newcommand{\productType}[2]{{\ensuremath{#1 \times #2}}}

%%% Contextual Modal Types
\newcommand{\contextualModalType}[2]{{\ensuremath{[#1 \vdash #2]}}}

%% CONTEXTS
\newcommand{\emptyContext}{\bullet}
\newcommand{\binding}[2]{#1 : #2}
% \newcommand{\lock}{\text{\upshape{[\!]}}}
\newcommand{\lock}{\text{\faLock}}

%% RELATIONS

\newcommand{\weakening}[2]{#1 \leq #2}
\newcommand{\contextMerge}[2]{#1 + #2}
%\newcommand{\typeDuality}[1]{\keyword{dualof}(#1)}
\newcommand{\typeDuality}[1]{{\overline{#1}}}
\newcommand{\subtyping}{\ensuremath{\leq}}

%% FUNCTIONS

\newcommand{\fv}[2]{\ensuremath{\keyword{FV}_{#1}(#2)}}
\newcommand{\dom}[1]{\ensuremath{\keyword{dom}(#1)}}
\newcommand{\tail}[1]{\keyword{tail}(#1)}
\newcommand{\countFun}[2]{\text{count(} #1 \text{,} #2 \text{)}}
\newcommand{\idFun}[1]{\text{id}_{#1}}
\newcommand{\upFun}[2]{#1 \uparrow #2}

%% TERMS

%% Terms Meta Variables
\newcommand{\constant}{c}
\newcommand{\evaluationContextVar}{E}

%%% Constants
\newcommand{\unit}{\keyword{unit}}
\newcommand{\integer}{\keyword{n}}
\newcommand{\true}{\keyword{true}}
\newcommand{\false}{\keyword{false}}

%%% Session Constants
\newcommand{\wait}{\keyword{wait}}
\newcommand{\close}{\keyword{close}}
%\newcommand{\skip}{\keyword{skip}}
\newcommand{\receive}{\keyword{receive}}
\newcommand{\send}{\keyword{send}}
\newcommand{\select}[1]{\keyword{select}\ #1}
\newcommand{\fork}{\keyword{fork}}
\newcommand{\fix}{\keyword{fix}}

%%% Lambda Calculus
%\newcommand{\abstraction}[3]{{\ensuremath{\lambda #1 . #3}}}
\newcommand{\abstraction}[3]{{\ensuremath{\lambda #1 ^{#2} . #3}}}
\newcommand{\application}[2]{{\ensuremath{#1 #2}}}
\newcommand{\pair}[2]{{\ensuremath{(#1, #2)}}}
\newcommand{\pairDestructor}[4]{{\ensuremath{\keyword{let}\ (#1, #2) = #3\ \keyword{in}\ #4}}}

%%% Session Terms
\newcommand{\new}[1]{{\ensuremath{\keyword{new}\ #1}}}
\newcommand{\match}[3]{{\ensuremath{\keyword{match}\ #1\ \keyword{with}\ \{#2\}^{#3}}}}

%%% Contextual Modal Type
\newcommand{\quo}[2]{{\ensuremath{\keyword{quo} \langle #1 \rangle #2}}}
\newcommand{\unq}[3]{{\ensuremath{\keyword{unq}_{#1} #2 [#3]}}}

%%% Evaluation Contexts

\newcommand{\hole}{[]}
\newcommand{\evaluationContextApply}[2]{#1 [#2]}

%% TYPE SYSTEMS

\newcommand{\typeof}[1]{\keyword{typeof}(#1)}
\newcommand{\isterm}[3]{\ensuremath{#1 \vdash #2 : #3}}
\newcommand{\stageTransition}[3]{\ensuremath{#1 : #2 \lhd #3}}
% \newcommand{\isun}[1]{#1~\operatorname{un}} No un types for the time being

%% SUBSTITUTIONS

\newcommand{\emptySubstitution}{\bullet}
\newcommand{\lockSubstitution}[1]{\lock_{#1}}
\newcommand{\singleSubstitution}[2]{#1 := #2}
\newcommand{\substitutionTyping}[3]{\ensuremath{\vdash #1 : #2 \Rightarrow #3}}

%% Evaluation Contexts

%% Operational Semantics

\newcommand{\reduction}[2]{\ensuremath{#1 \longrightarrow #2}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> packages/macros-theorems.tex <==
%% Macros for theorem and proofs

%% Several definitions for theorem-like environments
\newtheorem{corollary}{Corollary}
\newtheorem{convention}{Convention}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}

%% Numbering of environments relative to section
\numberwithin{corollary}{section}
\numberwithin{convention}{section}
\numberwithin{definition}{section}
\numberwithin{example}{section}
\numberwithin{lemma}{section}
\numberwithin{notation}{section}
\numberwithin{proposition}{section}
\numberwithin{remark}{section}
\numberwithin{theorem}{section}

%\newcounter{properties}
%\newtheorem{lemma}[properties]{Lemma}
%\newtheorem{theorem}[properties]{Theorem}
%\newtheorem{definition}[properties]{Definition}
%\newtheorem{proposition}[properties]{Proposition}


==> packages/macros-vasco.tex <==
% \newcommand{\ctxsep}{\text{[\!]}}

\definecolor{darkviolet}{rgb}{0.5,0,0.4}
\definecolor{darkgreen}{rgb}{0,0.4,0.2}
\definecolor{darkblue}{rgb}{0.1,0.1,0.9}
\definecolor{darkgrey}{rgb}{0.5,0.5,0.5}
\definecolor{lightblue}{rgb}{0.4,0.4,1}

\lstdefinestyle{eclipse}{
  breaklines=true,
  basicstyle=\sffamily\small,
  emphstyle=\color{red}\bfseries,
  keywordstyle=\color{darkviolet}\bfseries,
  commentstyle=\color{darkgreen},
  stringstyle=\color{darkblue},
  numberstyle=\color{darkgrey},%\lstfontfamily,
  emphstyle=\color{red},
  showstringspaces=false,
}

\lstset{
  language=Haskell,
  style=eclipse,
  morekeywords=[1]{Unit, Skip, Close, Wait, Dual, dualof, rec, new, close, wait, send,
    receive, select, fork, with, quo, unq},
  deletekeywords={all},
  % sensitive=true,
  literate=
  {->}{$\rightarrow$}2
  {-o}{$\multimap$}2
  {=>}{$\Rightarrow$}2 
  {forall}{$\forall$}1
  {Lambda}{$\Lambda$}1
  {lambda}{$\lambda$}1
  {mu}{$\mu$}1
  {alpha}{$\alpha$}1
  {oplus}{$\oplus$}1
  {+\{}{$\oplus$\{}2
  {vdash}{$\vdash$}2
  {<<}{$\langle$}1
  {>>}{$\rangle$}1
  {_0}{${_0}$}1
  {_1}{${_1}$}1
  {_k}{${_k}$}1
  {->^2}{${\rightarrow^2}$}2
  {->^3}{${\rightarrow^3}$}2
  {->^4}{${\rightarrow^4}$}2
  {->^5}{${\rightarrow^5}$}2
  ,
  breaklines=true,
  tabsize=2
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/figures/figure-local-completeness-arrow-un.tex <==
\begin{mathpar}
  \isterm{\ctxun{\Gamma}} M {\functionType T \multun U}
  %
  \quad\Rightarrow\quad
  %
  \inferrule*[right=\ruletsarrowuni]
  {
    \inferrule*[right=\ruletsarrowe]
    {
      \isterm{\ctxun{\Gamma}} M {\functionType T \multun U}
      \\
      \inferrule*[right=\ruletsvar]
      { }
      {\isterm{\binding{x}{(\contextualType{\emptyseq}{0}{T})}} {\appliedvar x \emptyseq} T}
    }
    {
      \isterm{\ctxun{\Gamma},\binding{x}{(\contextualType {\emptyseq}{0}{T})}} {\application M{\appliedvar x \emptyseq}} U
      % \\
      % \un{\Gamma}
    }
  }
  {\isterm{\ctxun{\Gamma}} {\abstraction x {} {(\application M{\appliedvar x \emptyseq})}} {\functionType T \multun U}}
\end{mathpar}


==> sections/figures/figure-local-completeness-box.tex <==

\textbf{Alternative.}
%
Take for $\tau$ the contextual type $\contextualType \emptyseq 1 U$ and for
$\Delta$ the unrestricted part of $\Gamma$. Then $\un U$ and
$\Gamma = \Gamma \csplit \Delta$.

\begin{mathpar}
\isterm {\Gamma} M {\contextualModalType\tau}
% 
\quad\Rightarrow\quad
%
\inferrule*[right=\ruletsboxe]
{
  \isterm {\Gamma} M {\contextualModalType\tau}
  \\
  \inferrule*[right=\ruletsboxi]
  {
    \inferrule*[right=\ruletsctxt]
    {
      \inferrule*[right=\ruletsvar]
      {
      }{
        \isterm{\Delta,\binding u \tau}{\appliedvar u \emptyseq}{U}
      }
    }{
      \isterm{\Delta,\binding u \tau}{\ctxval \emptyseq{\appliedvar u \emptyseq}}{\tau}
    }
  }{
    \isterm{\Delta,\binding u \tau}{\cbox{(\ctxval \emptyseq{\appliedvar u \emptyseq}})}{\contextualModalType\tau}
  }
}{
  \isterm{\Gamma}{\letbox u M {\cbox{(\ctxval \emptyseq{\appliedvar u \emptyseq}})}}{\contextualModalType\tau}
}
\end{mathpar}
%
This alternative works
\begin{itemize}
\item for any $\Gamma$
\item with the more general rule \ruletsboxe, as proposed by Yuito (not requiring $\ctxouter\Gamma n$)
\item with the current restriction $\ctxun\Gamma$ in rule \ruletsboxi
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> sections/figures/figure-local-soundness-arrow-un.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> sections/figures/figure-local-soundness-box.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> sections/figures/figure-local-soundness-pair.tex <==
\begin{mathpar}
\inferrule*[right=\ruletspaire]
{
  \inferrule*[right=\ruletspairi]
    {
      \isterm{\Gamma_1} {u}{T}
      \\
      \isterm{\Gamma_2} {v}{U}
    }
    {\isterm{\Gamma_1 \csplit \Gamma_2} {\pair{u}{v}}{\productType{T}{U}}}
    \\
    \isterm{\Delta,\binding x {T},\binding y {U}} {M}{V}
}
{\isterm{(\Gamma_1 \csplit \Gamma_2) \csplit \Delta}{\pairDestructor{x}{y}{\pair{u}{v}}{M}}{V}}
%
\quad\Rightarrow\quad
\end{mathpar}


\begin{equation*}
\begin{prooftree}
  \[
    \isterm{\Gamma_1}{u}{T}
    \justifies
    \isterm{\Gamma_1}{\ctxval{\emptyseq}{u}}{(\contextualType{\emptyseq}{0}{T})}
    \using \ruletsctxt
  \]
  \quad
  \[
    \[
      \isterm{\Gamma_2}{v}{U}
      \justifies
      \isterm{\Gamma_2}{\ctxval{\emptyseq}{v}}{(\contextualType{\emptyseq}{0}{U})}
      \using \ruletsctxt
    \]
    \isterm{\Delta,\binding x{T},\binding y{U}}{M}{V}
    \justifies
    \isterm{\Gamma_2 \csplit \Delta,\binding x{T}}{\substitution{\ctxval{\emptyseq}{v}}{y} M}{V}
    \using \rulesubs
  \]
\justifies
\isterm{(\Gamma_1 \csplit \Gamma_2) \csplit \Delta}{\substitution{\ctxval{\emptyseq}{u}}{x} \substitution{\ctxval{\emptyseq}{v}}{y} M}{V}
\using \rulesubs
\end{prooftree}
\end{equation*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> sections/proofs/proof-typing-contexts.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:

